A Scaling Law for Synthetic-to-Real Transfer: How Much Is Your Pre-training Effective?

Synthetic-to-real transfer learning is a framework in which a synthetically generated dataset is used to pre-train a model to improve its performance on real vision tasks. The most significant advantage of using synthetic images is that the ground-truth labels are automatically available, enabling unlimited expansion of the data size without human cost. However, synthetic data may have a huge domain gap, in which case increasing the data size does not improve the performance. How can we know that? In this study, we derive a simple scaling law that predicts the performance from the amount of pre-training data. By estimating the parameters of the law, we can judge whether we should increase the data or change the setting of image synthesis. Further, we analyze the theory of transfer learning by considering learning dynamics and confirm that the derived generalization bound is consistent with our empirical findings. We empirically validated our scaling law on various experimental settings of benchmark tasks, model sizes, and complexities of synthetic images.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:theory} and Appendix~\ref{sec:detail_theory}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{sec:detail_theory}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The training and evaluation scripts used for the experiments depends on proprietary libraries and we cannot publish them. Instead, we will publish the code for image rendering and pre-trained models. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec:train_details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See e.g. Figure~\ref{fig:complexity}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{sec:exp-setting}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See References.}
  \item Did you mention the license of the assets?
    \answerNA{We only use public libraries and benchmark data sets that do not require to mention the licence explicitly. }
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We will include scripts to generate synthetic images.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We only used publicly available data sets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We only used publicly available data sets and we believe these contents do not contain such concerns.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> method.tex <==
\section{Methods}

In this study, we employ the following protocol for transfer learning. First, we pre-train a model that consists of backbone and head networks until convergence, and we select the best model in terms of the validation error of the pre-training task. Then, we extract the backbone and add a new head to fine-tune all model parameters.  

For notations, let $L(n, s) \geq 0$ be the test error of a fine-tuning task with pre-training data size $n$ and fine-tuning data size $s$. The task names of object detection, semantic segmentation, multi-label classification, single-label classification, and surface normal estimation are abbreviated as \texttt{objdet}, \texttt{semseg}, \texttt{mulclass}, \texttt{sinclass}, and \texttt{normal}, respectively. The settings for transfer learning are denoted by arrows. For example, \transfer{objdet}{semseg} indicates that a pre-training task is object detection, and a fine-tuning task is semantic segmentation. 


\subsection{Deduction of scaling law} \label{sec:deduction}
%
\begin{wrapfigure}[9]{r}{0.5\textwidth}
  \vspace{-2em}  
  \begin{center}
    \includegraphics[width=0.23\textwidth]{img/example_pretrain.pdf}
    %\hspace{.05\textwidth}
    \includegraphics[width=0.23\textwidth]{img/example_finetune.pdf}
  \end{center}
  \caption{Asymmetric scaling. }
  \label{fig:example}  
\end{wrapfigure}
%
We make the following four requirements to formalize the scaling law. 
\begin{requirement}\label{asm:irr}
  The fine-tuning error is decomposed as $L(n,s) = \mathcal{R}(n,s) +  \mathcal{E}$, ($\mathcal{E}\geq 0$).
\end{requirement}
\begin{requirement}\label{asm:power}
  $\mathcal{R}(n,s)$ can be written as $\mathcal{R}(n,s)=f(n^{-\alpha}, s^{-\beta}) \geq 0$ with a simple function $f$.
\end{requirement}
\begin{requirement}\label{asm:finetune}
  $\lim_{s\to\infty} \mathcal{R}(n,s) = 0$.
\end{requirement}
\begin{requirement}\label{asm:pretrain}
  $\lim_{n\to\infty} \mathcal{R}(n,s) = \mathrm{const}$.
\end{requirement}

Requirements~\ref{asm:irr} and \ref{asm:power} follow the standard form of generalization given by the learning theory (e.g., PAC learning~\citep{mohri2018foundations}). Namely, the error is decomposed into reducible part $\mathcal{R}$ and irreducible parts $\mathcal{E}$ as $L(n,s) = \mathcal{R} +  \mathcal{E}$, where $\mathcal{R}$ depends on the polynomial decay with respect to the fine-tuning data size $s$. 
Further, we hypothesize that the effect of pre-training data size $n$ is embedded in the reducible part as a polynomial decay form, as pre-training helps reduce the fine-tuning error faster. 

Requirements~\ref{asm:finetune} and \ref{asm:pretrain} constrain how pre-training effect $n^{-\alpha}$ and fine-tuning effect  $s^{-\beta}$ interact with each other. When we fix the pre-training data size $n$ and increase the fine-tuning data size $s$, this is the case the standard scaling law~\citep{kaplan2020scaling} holds (pre-training only modifies initial weights). Hence the reducible error $\mathcal{R}$ should go to zero (Requirement~\ref{asm:finetune}). In contrast, when $s$ is fixed, $\mathcal{R}$ is not necessarily going to zero, especially when a pre-training task is largely irrelevant (Requirement~\ref{asm:pretrain}). Empirical results also support the asymmetry of the pre-training and fine-tuning effects.
%From the experiments in Section~\ref{sec:experiments}, an asymmetry of pre-training and fine-tuning is observed, and it plays a critical role in formulating the law.  By definition, $\mathcal{R}$ should go to zero as $s$ goes to infinity, whereas $\mathcal{R}$ does not necessarily go to zero as $n$ goes to zero.  This is observed when a pre-train task is largely irrelevant to a fine-tune task. 
%(e.g. pretraining MNIST for ImageNet classification). In that case, the pretraining effect is bounded and cannot push $\mathcal{R}$ to zero. 
%This asymmetry is clearly depicted in Figure~\ref{fig:example} (replicated from Figure~\ref{fig:fratio}). 
Figure~\ref{fig:example} (replicated from Figure~\ref{fig:fratio}) presents the log-log plot of scaling curves in the case of \transfer{mulclass}{sinclass} with respect to pre-training/fine-tuning data size, where each color indicates a different fine-tuning/pre-training data size. The left panel shows the pre-training effect diminishes for large $n$, while the right panel shows the fine-tuning effect follows a power law.

To satisfy Requirement~\ref{asm:finetune}, it is reasonable to formulate the law in a multiplicative form $\mathcal{R}(n,s) = g(n^{-\alpha})h(s^{-\beta})$ rather than the additive form $g(n^{-\alpha}) + h(s^{-\beta})$.
%, which has been derived as a generalization bound for transfer learning \cite{Maurer2016benefit}. 
In addition, a simple choice for Requirement~\ref{asm:pretrain} is to introduce an irreducible term as $g(n^{-\alpha}) \propto n^{-\alpha} + \gamma$ such that the effect of $n$ cannot be lower than $\gamma$.  By combining these, we obtain
\begin{align}\label{eq:full-law}
    L(n, s) = \delta (n^{-\alpha} + \gamma) s^{-\beta} + \mathcal{E},
\end{align}
where $\alpha,\beta>0$ are decay rates for pre-training and fine-tuning, respectively, $\gamma\geq 0$ is a constant, $\delta > 0$ is a coefficient, and $\mathcal{E} \geq 0$ is an optimal error that is irreducible owing to the noise. If we have sufficient observations, we can estimate these parameters by using the nonlinear least squares method. 
% While the derivation of \eqref{eq:full-law} here is empirical, we later show in Section~\ref{sec:theory} that the same form is derived from the theoretical analysis.

\paragraph{Simplification for empirical estimation}

When the number of observed points are limited in experimental studies, further simplification is necessary for numerical stability of empirical estimation. In particular, when $s$ is small (a standard setting of few-shot learning), it is not realistic to conduct experiments for many different $s$, and estimating all parameters in \eqref{eq:full-law} could be ill-conditioned. In this case, a practical solution is to simplify \eqref{eq:full-law} by eliminating $s$-dependent terms by setting $D=\delta s^{-\beta}$ and $C=\delta\gamma s^{-\beta} + \mathcal{E}$, which gives  \eqref{eq:simple-law}.
%\begin{align}\label{eq:simple-law-coef}
%    L(n, s) = D n^{-\alpha} + C
%\end{align}
Then, we can estimate $D$ and $C$ as they are independent parameters (rather than depending on $s$). We hereafter refer to \eqref{eq:full-law} as the full scaling law to distinguish from \eqref{eq:simple-law}.
%


\subsection{Experimental settings}\label{sec:exp-setting}
%We conducted the following experiments to study the scaling behaviors of transfer learning, and investigated whether the deduced \eq{eq:full-law} explains the results. 
The experiments were conducted on an in-house cluster containing NVIDIA V100 GPUs. The total amount of computation was approximately 1700 GPU days (200 for image rendering, 1300 for pre-training, and 200 for fine-tuning). Code and pre-trained models are available at \url{https://github.com/pfnet-research/cg-transfer}.

\paragraph{Pre-training data:} We generated synthetic image data sets by BlenderProc~\citep{denninger2019blenderproc}, an image renderer that can handle several domain randomization methods. For rendering, we used the setting of the BOP challenge 2020~\citep{hodan2020bop} as our default setting. We used 172 3D models, where ten objects appeared on average for each image. We applied texture randomization for walls and a floor, randomization for area and point lights, and randomization for the camera. Teacher signals (e.g., class labels for a classification task) were generated along with the images. We prepared two data sets of different sizes: 64 thousand and 1.28 million images. Because the learning curves of both data sets were similar, we showed the results of 64 thousand in the main paper and deferred the latter results in Appendix~\ref{sec:1280k}.

\paragraph{Pre-training:} We prepared four tasks: multi-label classification, object detection, semantic segmentation, and surface normal estimation. We used ResNet-based models, where backbones were ResNet-50, unless otherwise specified, and the head networks were customized for each task. We trained all models for the same fixed number of iterations depending on pre-training tasks and selected the best models as pre-trained models, which were validated by another 1000 synthetic images generated in the same way. 

\paragraph{Fine-tuning:} We employed three data sets: ImageNet (ILSVRC 2012)~\citep{ILSVRC15} for single-label classification, MS-COCO~\citep{lin2014microsoft} for object detection, and ADE20K~\citep{zhou2016semantic} for semantic segmentation. The number of images used was 1\% of each data set (roughly, 12 thousand for ImageNet, a thousand for COCO, and 2 hundred for ADE20K). We fine-tuned the pre-trained models with these subsets of data for a fixed number of iterations and reported the error metrics for validation sets at the last iteration. The metrics were top-1 accuracy for classification, mean mAP for MS-COCO, and mean IoU for ADE20K. These metrics take their values from 0 to 1, and we converted them into errors such as  1 - accuracy.

\paragraph{Curve fitting:} After obtaining the empirical errors, we estimated the parameters of \eqref{eq:simple-law} by nonlinear least squares in the log-log space, i.e., we solved the minimization problem $\min_{\alpha,C,D} \sum_i |\log \hat{L}(n_i, s) - \log(D n_i^{-\alpha} + C)|^2$ with a fixed fine-tuning data size $s$ and pre-training data sizes $n_i=2^i \times 1000$ for data point index $i=0,\dots,6$ where $\hat{L}$ denotes an observed error. Note that, except for the setting in Section~\ref{sec:fratio}, we fitted the curves independently for every different data sets, tasks, and $s$. All the results including Figure~\ref{fig:crosstask} were shown as log-log plots.

In the experiments, we empirically encountered some instability between $D$ and $\alpha$. We fixed $D=0.48$ by the median values of $D$'s for all the settings and estimated $\alpha$ and $C$ independently for each case. We explain this procedure with more details in Appendix~\ref{sec:illposedness}.  

%\subsection{Theoretical analysis of transfer}
%To investigate the scaling behaviors of transfer learning theoretically, we use the recent development for analysis of learning dynamics and generalization bounds of wide neural networks with the neural tangent  kernel \cite{NitandaSuzuki_ICLR2021optimal}, extending the results to transfer learning. Section \ref{sec:theory} will discuss the result in simple situations, which shows good agreement to the proposed law \eq{eq:full-law}. 

==> theory.tex <==
\section{Theoretical Analysis}\label{sec:theory}

This section provides a theoretical analysis of transfer learning in a simplified setting and derives a generalization bound, which agrees well with the full scaling law \eqref{eq:full-law}.  The analysis relies on the recent work on the convergence and generalization bounds by \citet{NitandaSuzuki_ICLR2021optimal}, and extends it to the case of the pre-training/fine-tuning scenario. The framework in \cite{NitandaSuzuki_ICLR2021optimal} is suitable for our purpose since we can consider the initialization of learning and do not need a lower bound of eigenvalue unlike \cite{arora2019finegrained}.  All details will be presented in Appendix~\ref{sec:detail_theory}.

In pre-training, the target function to learn is $\varphi_0$ with training data $(\tx_i,\ty_i)_{i=1}^{T_0}$, where $\tx_i\sim\rho_X$ is i.i.d.~and $\ty_i=\varphi_0(\tx_i)$.  In fine-tuning, the network is initialized by the parameter of the pre-training and the whole parameter is updated according to the stochastic gradient descent (SGD).  The target function in the fine-tuning is given by 
\begin{equation}
    \varphi(x) = \varphi_0(x) + \varphi_1(x),  
\end{equation}
To simplify the theoretical analysis, we assume noiseless training data, that is, the training data are given by $(x_j,y_j)_{j=1}^{T_1}$, where $x_i\sim \rho_X$ is i.i.d.~and $y_j = \varphi(x_j)$.  Also, we assume  $\|\tx_i\|_2=\|x_j\|_2=1$,  $\ty_i,y_j\in[0,1]$, and a simple scalar-valued two-layer neural network model:
\begin{equation}\textstyle{
    g_\Theta(x) = \frac{1}{\sqrt{M}} \sum_{r=1}^M a_r \sigma(b_r^T x),}
\end{equation}
where $\Theta=(a_r,b_r)$ is the parameter and the activation $\sigma$ is second differentiable so that $\sigma'$ and $\sigma''$ are bounded and $|\sigma(u)|\leq 1+|u|$.  We omit the bias term; however, with obvious modification, it is not difficult to include it.

Let $(\gamma_\ell)_{\ell=1}^\infty$ ($\gamma_1\geq \gamma_2\geq \cdots >0$)  denote the eigenvalues of the covariance operator $\Sigma_\infty:=E_{X\sim\rho_X}[k_\infty(\cdot,X)\otimes k_\infty(X,\cdot)^*]$, where $k_\infty$ is the neural tangent kernel \citep{Jacot_etal_NTK_NIPS2018,NitandaSuzuki_ICLR2021optimal}.
As the typical parameters for describing generalization bounds \cite{CaponnettoDeVito2007}, we assume (A1) there is $\xi > 1$ such that $\gamma_\ell \sim \ell^{-\xi}$, and (A2) there are $r_0,r_1\in[1/2,1]$ such that  $\varphi_i\in\mathcal{R}(\Sigma_\infty^{r_i})$ ($i=0,1$), where $\mathcal{R}$ denotes the range. The parameter $\xi$ represents the complexity of the hypothesis class $\cH_\infty$, which is the reproducing kernel Hilbert space  defined by $k_\infty$, and $r_i$ is the degree of smoothness of $\varphi_i$.  

As in \cite{NitandaSuzuki_ICLR2021optimal}, we consider the averaged SGD (ASGD), where one training sample $(x_t,y_t)$ is given at every time step for SGD, and the parameters $\Theta^{(0)},\ldots,\Theta^{(T)}$ are averaged to obtain the final result $\overline{\Theta}^{(T)}:=(T+1)^{-1}\sum_{t=0}^T \Theta^{(t)}$.  
For both the pre-training and fine-tuning, the objective function to minimize is the following regularized empirical risk:
\begin{equation}
\textstyle{
     L(\Theta):=\frac{1}{2}\sum_i (y_i - g_\Theta(x_i))^2 + \frac{\lambda}{2} \bigl\{ \|a-a^{(0)}\|_2^2 +  \sum_r \|b_r - b_r^{(0)}\|^2_2 \bigr\},
    }
\end{equation}
where $\Theta^{(0)} = (a_r^{(0)},b_r^{(0)})_{r=1}^M$ are the initial parameters for either the pre-training or fine-tuning, and $\lambda=\lambda_0$ and $\lambda_1$ are the regularization coefficients for pre-training and fine-tuning, respectively.

%For the pre-trainig, each  $b^{(0)}$ is independently given by the normal distribution $N(0,\kappa^2)$. As in \cite{NitandaSuzuki_ICLR2021optimal}, $a^{(0)}$ are initilized as $1$ or $-1$ so that $g_{\Theta^{(0)}}=0$.  The initial parameter of the fine-tune is the same as the final state of the pre-training. 
%
%At time step $t$ ($t\leq T$), one data $x_i$ is given by $\rho_X$ independently, and $(x_i,y_i)$ is used in the update rule:
%\begin{align}
%    \Theta^{(t+1)} = \Theta^{(t)} - \eta \frac{\partial L(\Theta^{(t)})}{\partial\Theta}
%\end{align}
%where $\eta$ is the learning coefficient, which is constant. More explicitly, 
%\begin{align}
%    a_r^{(t+1)}-a_r^{(0)} & = (1-\eta\lambda)(a_r^{(t)}-a_r^{(0)}) - \frac{\eta}{\sqrt{M}} (g_{\Theta^{(t)}} - y_t)\sigma(b_t^{(t)T}x_t), \nonumber \\
%    b_r^{(t+1)}-b_r^{(0)} & = (1-\eta\lambda)(b_r^{(t)}-b_r^{(0)}) - \frac{\eta}{\sqrt{M}} (g_{\Theta^{(t)}} - y_t)a_r\sigma'(b_t^{(t)T}x_t)x_t. 
%\end{align}
%After proceeding up to $T$ time step, the final parameter is given by 
%\begin{equation}
%    \overline{\Theta}^{(T)}:= \frac{1}{T+1} \sum_{t=0}^T \alpha_t \Theta^{(t)}. 
%\end{equation}
%The final network is given by the averaged parameter.

\citet{NitandaSuzuki_ICLR2021optimal} show that, if the regularization parameter is optimized, the ASGD for pre-training yields the generalization bound 
\begin{equation}\label{eq:bound_initial}
    \hat{R}_0:=E\|\hat{\varphi}_0 - \varphi_0\|^2_{L_2(\rho_X)} \leq c_M + A_0 T_0^{-\frac{2r_0\xi}{2r_0\xi+1}}\qquad (T_0\to\infty),
\end{equation}
where $\hat{\varphi}_0$ is the final network after $T_0$ data. The constant $c_M$ is arbitrarily small if $M\to\infty$, and $A_0$ is a constant factor that depends on $\varphi_0$. This bound is known to be of optimal rate in terms of $T_0$.

Extending \cite{NitandaSuzuki_ICLR2021optimal}, we obtain the bound of the  generalization error for transfer learning: 
\begin{thm}[Informal]\label{thm:bound_informal}
Suppose Assumptions (A1) and (A2) hold.  Fine-tune the network after pre-training that satisfies \eq{eq:bound_initial}. Then, for any $\varepsilon > 0$, there exists $M_0 \in \N$ such that for any $M \geq M_0$, the following holds with high probability:
\begin{align}
      E\|g_{\overline{\Theta}^{(T_1)}}- \varphi\|_{L^2(\rho_X)}^2  
      &\leq  \varepsilon + c_0 \lambda_1^{2r_0}+ c_1 \lambda_1^{2r_1}  + \frac{c_2}{T_1+1} \bigl\{ \lambda_1^{-1} \hat{R}_0 + a_{1,1}\lambda_1^{2r_1-1} + a_{1,2} \bigr\}  \nonumber \\
     &
    +\frac{c_3}{(T_1+1)^2\eta_1^2} \bigl\{ \lambda_1^{-2}  \hat{R}_0 + a_{2,1}\lambda_1^{2r_1-2} + a_{2,2}\lambda_1^{-1} \bigr\}
    + \frac{c_4}{T_1+1} \lambda_1^{-1/\xi},   
\label{eq:bound_informal}
\end{align}
where $\eta_1$ is a learning rate of ASGD, and constants $c_i,a_{i,k}$ depend on the function norms of $\varphi_0,\varphi_1$. 
\end{thm}
We consider the convergence rate for $T_1\to\infty$ with $\lambda_1$ and $\eta_1$ depending on $T_1$. We focus on the situation where the regularization $\lambda_1$ is larger than usual learning, reflecting the transfer learning setting, where the information of pre-training should be preserved.  Specifically, we assume $\lambda_1 = \Omega(T_1^{-\frac{2r_1\xi}{2r_1\xi+1}})$. In this case, the terms of rates $\lambda_1^{2r_0}$, $\lambda_1^{2r_1}$, $T_1^{-1}\lambda_1^{-1}$, and  $T_1^{-2}\eta_1^{-2}\lambda_1^{-2}$ can be dominant.  

Among the possible cases discussed in Section \ref{sec:theory-rates}, we here show the convergence rate only for $r_0\geq r_1$ and $\eta=T_1^{-\zeta}$ with $\zeta\in[\max\{r_1/(2r_1+1),(r_1\xi+1-\xi)/(2r_1\xi+1)\},1]$. Details and the other cases are shown in Appendix~\ref{sec:detail_theory}.  By equating two dominant terms  $\lambda_1^{2r_1}$ and $T_1^{-2}\eta_1^{-2}\lambda_1^{-2}$, $\lambda_1 = T_1^{-(1-\zeta)/(r_1+1)}\hat{R}_0^{1/(2r_1+2)}$ is optimal and 
\begin{equation}\label{eq:main_bound_0}
\textstyle{
    E\|g_{\overline{\Theta}^{(T_1)}}- \varphi\|_{L^2(\rho_X)}^2  \leq \varepsilon + C T_1^{-\frac{2r_1(1-\zeta)}{r_1+1}}\hat{R}_0^{\frac{2r_1}{2r_1+2}}.
}
\end{equation}
Although the current learning method is online-type, different from the one used in the previous sections, based on the fact that the ASGD achieves the optimal learning rate, we match the data size as $T_0=n$ and $T_1=s$.  Plugging \eq{eq:bound_initial} into \eq{eq:main_bound_0}, we obtain 
\begin{equation}\label{eq:main_bound}
        E\|g_{\overline{\Theta}^{(T_1)}}- \varphi\|_{L^2(\rho_X)}^2  \leq \varepsilon + C(c'_M + A'_0 n^{-\frac{2r_0\xi}{2r_0\xi+1}\cdot\frac{r_1}{r_1+1}})s^{-\frac{2r_1(1-\zeta)}{r_1+1}}.
\end{equation}
It is notable that \eq{eq:main_bound} has the same form as the proposed scaling law \eqref{eq:full-law}.  This provides theoretical support to the law, while the problem settings are not exactly the same.   Since $r_1\in[1/2,1]$, with a large value of $r_0\xi$, the exponent of $T_0$ ranges roughly in $[-1/2,-1/3]$.
%Note that if $\zeta=(r_1\xi+1-\xi)/(2r_1\xi+1)$, the optimal convergence rate $T_1^{-\frac{2\xi r_1}{2\xi r_1+1}}$ with respect to $T_1$ is recovered.  \eq{eq:main_bound} is the same as the proposed form of the scaling law \eq{eq:full-law}.  Since $r_1\in[1/2,1]$, with a large value of $r_0\xi$, the exponent of $T_0$ ranges roughly in $[-1/2,-1/3]$.
%, and for large $r_0\xi$ it is close to $1/2$.  This shows a remarkable accordance with the estimate of $\alpha$ in Section \ref{sec:fratio}.    



